A Unified Iteration Space Transformation Framework for Sparse and Dense Tensor Algebra

We address the problem of optimizing mixed sparse and dense tensor algebra in a compiler. We show that standard loop transformations, such as strip-mining, tiling, collapsing, parallelization and vectorization, can be applied to irregular loops over sparse iteration spaces. We also show how these transformations can be applied to the contiguous value arrays of sparse tensor data structures, which we call their position space, to unlock load-balanced tiling and parallelism. We have prototyped these concepts in the open-source TACO system, where they are exposed as a scheduling API similar to the Halide domain-specific language for dense computations. Using this scheduling API, we show how to optimize mixed sparse/dense tensor algebra expressions, how to generate load-balanced code by scheduling sparse tensor algebra in position space, and how to generate sparse tensor algebra GPU code. Our evaluation shows that our transformations let us generate good code that is competitive with many hand-optimized implementations from the literature.

==> Makefile <==
pdf: main.pdf
.PHONY: pdf

main.pdf: 
	latexmk -pdf main.tex
.PHONY: main.pdf

notodo:
	latexmk -pdf -pdflatex='pdflatex %O -interaction=nonstopmode -synctex=1 "\def\notodo{1}\input{%S}"'main.tex
.PHONY: notodo

main.ps: main.pdf
	acroread -toPostScript $<

clean:
	latexmk -C main.tex
	rm -f *.bbl *.log
.PHONY: clean

view: main.pdf
	open main.pdf
.PHONY: view

skim: main.pdf
	open -a "Skim" main.pdf
.PHONY: skim

safe: main.pdf
	mkdir -p archive
	cp $^ archive/`date "+%y.%m.%d-%H.%M.%S"`-`openssl md5 < $^`.pdf

SPELLTEX := $(shell ./bin/get-tex-files.sh main.tex)
spell:
	@ for i in $(SPELLTEX); do aspell --mode=tex -p ./aspell.words -c $$i; done
	@ for i in $(SPELLTEX); do perl bin/double.pl $$i; done
	@ for i in $(SPELLTEX); do perl bin/abbrv.pl  $$i; done
	@ bash bin/hyphens.sh $(SPELLTEX)
	@ ( head -1 aspell.words ; tail -n +2 aspell.words | sort ) > aspell.words~
	@ mv aspell.words~ aspell.words
.PHONY: spell



==> iteration-space-transformations.tex <==
In this section, we will describe a transformation framework for
sparse, dense, and mixed sparse/dense iteration spaces.  The
framework operates on an intermediate representation called
iteration graphs, that extend the iteration graphs described by
Kjolstad et al.~\cite{kjolstad2017}.  The iteration graphs
describe the lexicographically ordered sparse iteration space that
results from iterating over hierarchical coordinate hierarchy
tensor data structures, and transformations on the graphs
transforms that space.  Combined with iteration graph code
generation, described in the next section, we can create loop
nests that iterate over the space by coiterating over coordinate
hierarchies.

\TODO{Summary of transformations}

\subsection{Iteration Graph Background}

\TODO{Move iteration graphs to its own section?}

We can symbolically describe an iteration space by a
lexicographical ordering of index variables that represent
dimensions, as in the polyhedral model.  We extend this to a tree
of such variables, where the concatenated ranges of the variables
of each tree level together encode a dimension.  This is analogous
to an imperfect loop nest where an outer loop contains two or more
sequenced loops.  These index variable trees describe the full, or
dense, iteration space of a tensor algebra expression.

Sparse iteration graphs extend iteration variable trees with paths
through the index variable nodes that each represent a coordinate
tree hierarcy that encode a subset of the iteration space.  In
tensor algebra these coordinate hierarchies, as we saw in the
previous section, come from the data structures that encode the
nonzero values of tensors.  \figref{iteration-graphs} (left) shows
two abstract coordinate hierarchies for the matrix-vector
multiplication example.  The expression has two index variables
and we chose to lexicographically order $i$ before $j$.
\figref{iteration-graphs} (middle) shows the two symbolic paths
induced by these hierarchies.  The matrix $B$ enumerates both $i$
and $j$ coordinates and therefore its path go through both
variables, whereas the vector $c$ only enumerates $j$ coordinates.
Finally, \figref{iteration-graphs} (right) shows the iteration
graph that contains both paths, since the whole expression must
coiterate over both coordinate hierarchies.  Note that the graph
is annotated with an intersection operation between the two paths
incoming on $j$.  This means the iteration space of $j$ is the
intersection of each row of $B$ and the vector $c$.  It is an
intersection because multiplying any variable by zero yields a
zero.  It is therefore sufficient to iterate over those
coordinates where both operands have a value to compute the
expression's nonzeros.  Conversely, a tensor addition would induce
a union between incomming paths.


\subsection{Derived Index Variables and Provenance Graphs}

In this paper, we further iteration graphs with the concepts of
\textbf{derived index variables}.  These are new dimensions that
are added to an expression's iteration space by the split, fuse,
and position iteration space transformations and can be in
coordinate space or position space.  The relationships between
derived index variables and the original index variables, that
index into tensors, are tracked by an \textbf{index variable
provenance graph}.  Provenance graphs let us map between the
transformed iteration space and the original space, so that the
code generator of the next section can compute the coordinates in
the original space that are used to index into tensors.

\begin{figure}[]
    \centering
    \begin{tabular}{m{1em} c c c}
    & Iteration Graph & Nested Iteration & Unrolled Iteration \\
    Original &
    \includegraphics[width=.05\linewidth]{figures/tiling-untiled-iteration-graph}  &
    \includegraphics[width=.40\linewidth]{figures/tiling-untiled-nested-iteration}  &
    \includegraphics[width=.40\linewidth]{figures/tiling-untiled-unrolled-iteration} \\
    Tiled &
    \includegraphics[width=.05\linewidth]{figures/tiling-tiled-iteration-graph}  &
    \includegraphics[width=.40\linewidth]{figures/tiling-tiled-nested-iteration}  &
    \includegraphics[width=.40\linewidth]{figures/tiling-tiled-unrolled-iteration}  \\
    \end{tabular}
    \caption{Iteration graphs, nested iteration orderings, and unrolled iteration orderings are shown for an untiled row-major iteration (top) and a tiled iteration (bottom).}
    \label{fig:tiledigraph}
\end{figure}

\TODO{Provenance graphs here?}


\subsection{Coordinate and Position Transformations}

The \code{coord} and \code{pos} transformations
create new index variables in the coordinate and position spaces
from index variables in the position and coordinate spaces
respectively.  Specifically, the \code{pos} transformation takes a
index variable in the coordinate space and replaces it with a new
derived index variable that operates over the same iteration
range, but with respect to one input's position space.  The
\code{coord} transformation, on the other hand, takes an index
variable in position space and replaces it with a new derived
dimensional iterator that iterates over the corresponding
iteration range in the coordinate iteration space.


\subsection{Reorder}

The \code{reorder} transformation interchanges two
directly nested index variables in an iteration graph.  This
changes the order of iteration through the space and the order of
tensor accesses.  The precondition of a reorder transformations is
that it does not hoist a tensor operation outside a reduction that
it does not distribute over.  \TODO{figure ...}

\begin{figure}[]
    \centering
    \includegraphics[width=.4\textwidth]{figures/space-transformations}
    \caption {
      An original row-major nested iteration of a two-dimensional
      coordinate iteration space is shown alongside various
      transformed nested iterations caused by different iteration
      space transformations.
    }
    \label{fig:spacetransformations}
\end{figure}


\subsection{Fuse}

The \code{fuse} transformation collapses two directly nested index
variables in an iteration graph.  It results in a new fused index
variable that iterates over the product of the coordinates of the
fused index variables.  This transformation by itself does not
change iteration order, but facilitates other transformations such
as iterating over the position space of several variables and
distributing a multi-dimensional loop nest across a thread array
on GPUs.  \TODO{figure ...}


\subsection{Split}

The \code{split} transformation splits (strip-mines) an index
variable into two nested index variables, where the size of the
inner index variable is constant.  The size of the outer index
variable is the size of the original index variable divided by the
size of the inner index variable, and the product of the new index
variables sizes therefore equals the size of the original index
variable.  Note that in the generated code, when the size of the
inner index variable does not perfectly divide the original index
variable, a tail strategy is employed such as emitting a variable
sized loop that handles remaining iterations.  \TODO{figure ...}


\subsection{Divide}

The \code{divide} transformation splits one index variable into
two nested index variables, where the size of the \emph{outer}
index variable is constant.  The size of the inner index variable
is thus the size of the original index variable divided by the
size of the outer index variable.  The \code{divide}
transformation is important in sparse codes because locating the
starting point of a tile can require a $O(n)$ or $O(\log (n))$
search.  Therefore, if we want to parallelize a blocked
loop, then we want a fixed number of blocks and not a number that
varies with the size of the tensor.


\subsection{Parallelize}

Finally, the \code{parallelize} transformation tags an index
variable for parallel execution.  That is, the resulting
iteration, or loops, will be executed in parallel.  The
transformation takes as an argument the type of parallel hardware
to execute on, such as CPU threads, a GPU thread array, or a SIMD
unit.  Parallelizing the iteration over an index changes the
iteration order of the loop, and therefore requires reductions
inside the iteration space described by the index variable's
sub-tree in the iteration graph to be associative.  Furthermore,
if the computation uses a reduction strategy that do not preserve
the order, such as atomic instructions, then the reductions must
also be commutative.



\HIDE {
\clearpage

\begin{figure*}[]
    \centering
    \includegraphics[width=.7\textwidth]{"PLDI Figures - Page 6".jpg}
    \caption{Iteration graphs, nested iteration orderings, and unrolled iteration orderings are shown for an untiled row-major iteration (top) and a tiled iteration (bottom).}
    \label{fig:tiledigraph}
\end{figure*}

To generate code from a tiled coordinate iteration space, we need to order the iteration of tiles into loop nests. Iteration graphs, first introduced in \ref{}, are an intermediate representation for the hierarchical dimensional ordering that an iteration space is iterated.  We extend this concept with \textbf{derived dimensional iterators}, which allow us to express the order that a tiled or fused dimension is iterated in. In Figure \ref{fig:tiledigraph}, we provide an example iteration graph before and after the iteration space is tiled. By constructing additional nodes in the iteration graph, we are able to express complex nested iterations, which create complex unrolled iteration patterns. In addition to allowing the translation of any existing iteration space to an iteration graph, we also provide a set of transformations that operate on the iteration graph directly and allows tiling of the coordinate iteration and position spaces. By expressing transformations directly on the iteration graph, we track how the loop nests change after each tiling while still allowing the user to conceptualize the transformations as tilings of the coordinate iteration space.

A sparse iteration graph is a tree embedding of a directed graph that represents a sparse iteration space. Each graph node is one of the dimensions of the space and is named by the index variable that iterate over it. The tree embedding of the graph orders the nodes in a tree structure, with ordered siblings, that describes the order of the iteration through dimensions. To express tiled iterations, we allow graph nodes to contain index variables that do not appear as dimensions in the original iteration space. These derived index variables have relationships to the original underived index variables and the underived variables can be recovered during iteration as we will show in Section \ref{sec:compiling}.

A sparse iteration graph only specifies the order that points in the iteration space are iterated in and not how they are iterated. For sparse loops, it is often more efficient to directly coiterate the input datastructures rather than enumerate all possible values in the iteration space and then check if the inputs are valid at this iteration point. Any such coiteration is a valid lowering of a given iteration graph as long as any nonzero points are iterated in the order specified by the iteration graph. Derived index variables can also be in position space as the mapping between a given position space and coordinate space is just another type of relationship that can be reversed to recover the underived variables. However, this does not mean that an iteration of the position space will occur at this iteration graph node. An index variable being in position space does not change the order of iteration by itself, but can be combined with other tiling operations to allow for different iteration orders that tile position space.

Transformations on the iteration graph can reorder existing nodes, construct new derived dimensional iterator nodes, and remove existing nodes. All transformations ensure that the property that all points in the iteration space are visited exactly once is maintained. Additionally information about how to relate new derived dimensional iterators to the original underived dimensional iterators is maintained in a separate datastructure discussed in Section \ref{relgraph}. 

In Figure \ref{fig:spacetransformations}, we show the effect that the transformations Split, Fuse, and Reorder have on the nested iteration order of a row-major iteration of a two dimensional iteration space. These transformations operate the same as in Halide on dense spaces and we will show how they extend to sparse spaces. 
\begin{itemize}
\item The $\mathbf{Split_{size}}$ transformation splits a single dimensional iterator into new outer and inner derived dimensional iterator. The inner iterator is of fixed length $size$ and the outer iterator iterates over all inner iterators such that the original dimension is fully iterated over. This transformation also operates differently depending on a tail strategy, which handles when the dimension's length is not evenly divisible by $size$.
\item The \textbf{Reorder} transformation reorders existing dimensional iterators in any arbitrary nesting order. In the context of sparse tensor algebra, the ordering of dimensions can result in asymptotically different performance. Additionally, while other space transformations can construct new derived dimensional iterators, the actual ordering of points in the iteration space can only change after these derived iterators are reordered.
\item The \textbf{Fuse} transformation replaces two directly nested dimensional iterators with a single new derived dimensional iterator that iterates over all points that the original nested iteration would iterate over. This transformation by itself does not change the iteration order, but can allow for splitting up an iteration along multiple dimensions at once.
\end{itemize}

\begin{figure}[]
    \centering
    \includegraphics[width=.4\textwidth]{figures/space-transformations}
    \caption{An original row-major nested iteration of a two-dimensional coordinate iteration space is shown alongside various transformed nested iterations caused by different iteration space transformations.}
    \label{fig:spacetransformations}
\end{figure}

These transformations operate the same way over position domains, which allows efficiently transforming sparse iteration spaces. Fusing iterators with respect to the position space creates a new derived iterator that iterates over all nonzero points in the fused iteration with respect to a given input. This allows for representing hierarchy tiling operations as discussed in Section \ref{sec:positionspace}. Similarly, splitting an iterator in position domain allows for creating iteration ranges with the same number of nonzero points with respect to a single input. We provide two new transformations to allow for moving back and forth between scheduling coordinate and position domain.

\begin{itemize}
\item The \textbf{Pos} transformation takes a dimensional iterator in coordinate space and replaces it with a new derived dimensional iterator that operates over the same iteration range with respect to one input's position space.
\item The \textbf{Coord} transformation takes a dimensional iteration in position space and replaces it with a new derived dimensional iterator that iterates over the corresponding iteration range in the coordinate iteration space.
\end{itemize}

Splitting sparse iteration spaces into separate ranges may cause for an overhead proportional to the number of ranges. This overhead is caused by the lack of random-access for the start location of a given iteration range and for an input dimension of size $n$, each iteration range could cause for a $\Theta(log(n))$ or even $\Theta(n)$ overhead depending on how the inputs are stored in memory. For dense computations, that need to be tiled for parallelism or data locality, we can create $\Theta(n)$ tiles, but using this strategy on a sparse iteration space could cause for asymptotically worse performance.

To allow for transforming computations into tiles such that this transformation does not asymptotically worsen the performance, we also provide the $\mathbf{Divide_{size}}$ transformation. This transformation is similar to $Split$ in that it creates two derived dimensional iterators that iterate over the points of a single dimensional iterator, but instead of the size of each iteration range being fixed, the number of iteration ranges is fixed to $size$. This means that the range of the outer dimensional iterator is of fixed size, while the the inner dimensional iterator's size will change depending on the size of the original dimensional iterator. This ensures a constant overhead regardless of original input size. A common misconception is that $Divide$ is simply $Split$ and then $Reorder$. However, these two transformations cause for a strided iteration, while $Divide$ creates a fixed number of contiguous iterations.

Iteration graphs and derived dimensional iterators provide a convenient representation for tracking the ordering of a nested iteration and allow us to reason about transforming coordinate iteration and position spaces with respect to the order that they will be iterated. They also allow us to largely ignore sparse coiteration of datastructures while transforming this space, which can create many different loops and cases. Iteration graphs provide a clean, easily-transformable intermediate representation that are also more readily representable to users so that they can check transformations of their program without understanding the more complicated generated code. In the next section, we will discuss how iteration graphs are also easily lowered to code targeted to different parallel architectures.

}

